Borinot: an agile torque-controlled robot for hybrid flying and contact loco-manipulation (workshop version)

This paper introduces Borinot, an open-source flying robotic platform designed to perform hybrid agile locomotion and manipulation. This platform features a compact and powerful hexarotor that can be outfitted with torque-actuated extremities of diverse architecture, allowing for whole-body dynamic control. As a result, Borinot can perform agile tasks such as aggressive or acrobatic maneuvers with the participation of the whole-body dynamics. The extremities attached to Borinot can be utilized in various ways; during contact, they can be used as legs to create contact-based locomotion, or as arms to manipulate objects. In free flight, they can be used as tails to contribute to dynamics, mimicking the movements of many animals. This allows for any hybridization of these dynamic modes, like the jump-flight of chicken and locusts, making Borinot an ideal open-source platform for research on hybrid aerial-contact agile motion. To demonstrate the key capabilities of Borinot, we have fitted a planar 2DoF arm and implemented whole-body torque-level model-predictive-control. The result is a capable and adaptable platform that, we believe, opens up new avenues of research in the field of agile robotics.

==> sections/discussion.tex <==
\section{Discussion}

\comment{What is missing to the current design, its drawbacks and possible future work.}

\comment{We have seen that the arm can help a lot in the general locomotion of the robot. Currently, the arm can only help in the X direction. Thus, we should think of other arm designs that allow the arm to also help in the other directions.}

==> sections/robot_overview.tex <==
\section{Borinot overview}

\cb{Do we need to introduce some notation/background/frames here?}

\comment{
  We should go from general structure to details. That is, we have two main parts, the platform, and the arm. For each part we should comment on the following general aspects:
\begin{itemize}
  \item Hardware and structural elements composing the assembly (this might be a good point to refer to a figure and comment on the weights).
  \item If there is any special reason why the structure, the assembly, and the element distribution have been created the way it is, it should be explained here. For example, 
  \item Explain more in detail of the sub-parts: power train system, battery, flight controller, onboard computer, etc.
  \item Hardware interfaces (how each element is connected to the other).
\end{itemize}
}

The Borinot robot (bumblebee in Catalan) is composed of two main parts: a hexacopter flying platform, and a robotic arm.
In the following, we give a detailed overview of both subsystems.

\subsection{Hexacopter platform}
The Borinot hexacopter (shown in \figref{fig:ro_platform_overview}) has been designed to be compact and small (its diagonal distance is of $370 \si{\milli\meter}$).
\todo{Why a hexacopter. This should be defended here.}
This allows its use in small-sized robotics laboratories.
Its structure is composed of six carbon fiber tubes of $\varnothing 8 \times \varnothing 6 \si{\milli\meter}$ of $270\si{\milli\meter}$ and $310\si{\milli\meter}$ \todo{check length} long.
They form two independent equilateral triangles that are placed in opposition to form a hexagon with a $370 \si{\milli\meter}$ diagonal (distance between the rotation axes of opposed motors).
This unusual configuration provides the platform with high rigidity and low weight \todo{see table with weights} 
\comment{Should we do any test to prove the rigidity claim?}.
The carbon fiber tubes as well as the rest of the components are held together by 3D-printed parts and regular M3 screws.
Provided that the carbon fiber tubes are already cut at the specified length, the platform can be manufactured using only a 3D printer and common tools such as a soldering iron, Allen keys, and a set of pliers.

\begin{figure*}[t]
  \centering
  \includegraphics{figures/borinot_exploded.eps}
  \caption{Exploded view of the Borinot hexacopter. \todo{This figure has to be done properly once Patrick finishes the redesign. Better colors, properly exploded, label on components, probably smaller, etc.}}
  \label{fig:ro_platform_overview}
\end{figure*}


\begin{table}[t]
  \caption{Weight list of the grouped by component type \todo{finish the table with the real weights and include all parts from the platform and the arm.}}
  \label{tab:ro_weight_list}
  \begin{center}
    \begin{tabular}{@{}l c c@{}}
      \toprule
      & \textsc{Weight $[\si{\gram}]$} & \textsc{Cost (approx.) [\texteuro]} \\
      \midrule
      \textsc{Structural parts} \\
      Carbon fiber tubes & 25 \\ 
      Screws and nuts & 54 \\
      \midrule
      \textsc{3D printed parts} \\
      Motor mounts & 120 \\
      NUC holder &   230 \\
      Other parts &   230 \\
      \midrule
      \textsc{Drive system} \\
      TMotor F90 1300KV & 120 \\
      TMotor F35A &   230 \\
      Cables and connector &   230 \\
      \midrule
      \textbf{\textsc{Total}} \\
      \bottomrule
    \end{tabular}
  \end{center}
\end{table}

\todo{Add here a comment regarding the final position of the center of mass. Both with an arm and without an arm. We should do this since we added this fact as a requirement}

The Borinot flying platform holds different subsystems:
\begin{enumerate}
  \item the power and drive systems, which is composed of the motors, the\glspl{esc} and the battery, which is used to supply energy to all the robot's subsystems
  \item the flight controller, which is used to cope with the functionalities related to flying such as the state estimation of the platform, the communication with a radio control transmitter-receiver system or the writing to the \glspl{esc}.
  \item the onboard computer that is used to run the algorithms that operate the robot.
\end{enumerate}

\subsubsection{Power \& Drive system}
As pointed out in \secref{subsec:int_requirements}, the platform's agility is enabled by a high \gls{twr}, which allows quick attitude changes.
% we have pointed out the need for a high \gls{twr} (higher than $3$ \todo{Why 3?}) \todo{Refer to the exact requirement in \secref{subsec:int_requirements}}.
To achieve that, we should keep a low weight (see \tabref{tab:ro_weight_list}) and find motors that give us a reasonable amount of thrust.
In the past recent years,  the range of available \gls{bldc} motors for multicopters has increased significantly leading to motors with special characteristics depending on the field of application (\gls{fpv}, aerial photography and cinema, surveillance, etc.). 

\begin{figure}[t]
  \centering
  % \includesvg{figures/2_control_architecture}
  \includegraphics[width=\columnwidth]{figures/borinot_layout.pdf}
  \caption{Borinot's power distribution scheme.}
  \label{fig:ro_power_distribution}
\end{figure}

The dimensions of our platform constrain the size of the propellers, which cannot be higher than $7$ inches.
Thus, we target motors that are mainly used within the \gls{fpv} community, which typically uses small-sized propellers.
The selected \textsc{TMotors F90-1300KV} \cite{tmotor_datasheet} are suited for 2-blade 7-inch propellers with great thrust capability.
These motors, powered by a $6\text{S}$ battery and equipped with a 7-inch propeller with 4.2 inches pitch can produce up to $20\si{\newton}$ of thrust ($120\si{\newton}$ in total). In \secref{subsec:exp_motor} one can find more data related to the performance of this motor.

The motor selection highly restricts the characteristics of the \glspl{esc} and the battery.
The selected \gls{esc} is the \textsc{TMotor F35A 6s}, which is a drone racing component that allows to operate of the motor with a $6S$ battery and a fast throttle response.
In addition, we have selected a $6\text{S}$ battery (nominal $22.2\si{\volt}$), with $3\si{\ampere\hour}$ and a discharge rate of $60\text{C}$.
This selection gives enough room to continuously operate the drone at the $85\%$ of its throttle capacity and have burst loads up to the $100\%$.

\comment{

COMMENTS:
\begin{itemize}
  \item Be aware that throttle capacity (one single motor) is not the same as thrust capacity (all the platform), we might want to translate everything in terms of thrust capacity.
  \item Should we add some autonomy numbers here, or should we add them in the experiment section?
\end{itemize}  
}

\todo{Be sure of these numbers and what they imply, for example, in terms of temperature. theoretically these should be bearable by the ESCs and the battery, but I'm not sure about the motors and whether they will become too hot.}

\subsubsection{Flight controller}
The flight controller selection is usually tied to the type of firmware that we want to use.
We have opted for a flight controller that is compliant with the PX4 flight stack (see the justification of this choice in \secref{subsec:so_px4}).

From the whole spectrum of flight controllers compatible with the PX4 firmware, we have opted for those that have an ethernet adapter, which enables for fast communication between the flight controller and the onboard computer.
In particular, we have used the \textsc{Holybro Pixhawk 5X}.

\comment{Not sure if we should add more info about this controller (like sensor or communication capabilities) or this is enough and we can refer the reader to the datasheet.}

\subsubsection{Onboard computer}
The Borinot mounts an Intel NUCi7DNKE, which mounts an Intel i7-8650U with 4 cores and a clock frequency of $1.9\si{\giga\hertz}$ and $32\si{\giga\byte}$ of DDR4 RAM.
This computer enables the use of computation-intensive controllers, such as \gls{mpc}.
\comment{This processor benchmarks 6303 at cpubenchmark. This website is used at Agilicoious paper to classify research multicopters according to its CPU marks. They do a plot classifying the platforms according to their \gls{twr} and the CPU benchmark. According to this classification, we equal the  \gls{twr} to that of Agilicious and we have a much higher cpubenchmark (6303 vs. 1343). We might want to cautiously make a claim here, stating that we offer a platform with the same \gls{twr} and much higher CPU mark.}

Besides, as this is a computer with bigger footprint than the ones that are typically mounted in aerial vehicles \cite{foehn_AgiliciousOpensourceOpenhardware_2022}, there is room in case any user wants to mount, \eg, a lighter computer.

\subsection{Odri-based arm}
To comply with the requirements in \secref{subsec:int_requirements} that affect the arm, we have chosen to use the \gls{odri} ecosystem \cite{grimminger_OpenTorqueControlledModular_2020}.
This initiative proposes an open-source robotic actuator (electronic and mechanical parts) that enables the build of affordable agile legged robots such as quadrupeds or bipeds.
Therefore, we have chosen a technology to build arms rather than a specific arm design for an agile aerial robot.

In fact, it is difficult to propose an arm design that could serve any task.
Typically, this problem is tackled by adding multiple \glspl{dof} (usually, more than $5$).
However, in this work we propose to explore a different approach.
On the one hand, we approach tasks from an agile point of view.
\comment{explain better: "that is, ...."}
This allows to do tasks while the platform is in an unstable pose, hence enlarging the operational space of the arm (see \secref{subsubsec:agile_end_effector}).
On the other hand, instead of an \emph{all-in-one} arm design, which would add excessive weight to the robot and it would compromise its agility, we opt for arm designs tailored to each specific application.
Thus, we have provided a mechanical interface in Borinot's platform to quickly change the arm of the robot (see \figref{fig:ro_arm_design}).

\begin{figure}[t]
  \centering
  % \includesvg{figures/2_control_architecture}
  \includegraphics[width=\columnwidth]{example-image-a}
  \caption{Borinot's $2$-\gls{dof} arm, with a weight on its end-effector to help in the agile flying locomotion.}
  \label{fig:ro_arm_design}
\end{figure}

In this work, we present a planar $2$-\gls{dof} arm (see \figref{fig:ro_arm_design}).
In order to keep the weight as close as possible to the platform and to ensure a small footprint, we have designed a new arm's base link that contains the same hardware parts as the \gls{odri} actuator.
For the second link we have used a Solo12 leg.
\comment{Any comment on the nut helping the locomotion?}

The electronics of the arm are composed of the master board, which handles the communication with the on-board computer and the uDriver, that is in charge to drive the two motors. 
Both electronic boards are placed next to the base link and close to the platform.


==> sections/software_overview.tex <==
\section{Software}

\subsection{Flight controller firmware: PX4}
\label{subsec:so_px4}
\begin{itemize}
  \item Why have we chosen the PX4 stack?
  \begin{itemize}
    \item Popularity within the community. It is a widely adopted system.
    \item Tested system as a backup:
    \begin{itemize}
      \item Tested controllers as a backup
      \item Off-the-shelf state estimation system that enables fusion with mo-cap
      \item Fast communication with an on-board computer (in its 5x and 6x version, with ethernet communication)
      \item Thoroughly tested auxiliary systems to operate a multicopter-based vehicle: flight mode machinery, RC remote control, ROS2 communication ready. 
    \end{itemize}
  \end{itemize}
\end{itemize}
\todo{Explain the modifications we have done to the base firmware.}


\subsection{Robot Operating System: the Eagle ROS2 package}



